Semantic Parsing in Task-Oriented Dialog with Recursive Insertion-based Encoder

We introduce a Recursive INsertion-based Encoder (RINE), a novel approach for semantic parsing in task-oriented dialog. Our model consists of an encoder network that incrementally builds the semantic parse tree by predicting the non-terminal label and its positions in the linearized tree. At the generation time, the model constructs the semantic parse tree by recursively inserting the predicted non-terminal labels at the predicted positions until termination. RINE achieves state-of-the-art exact match accuracy on low- and high-resource versions of the conversational semantic parsing benchmark TOP (Gupta et al., 2018; Chen et al., 2020), outperforming strong sequence-to-sequence models and transition-based parsers. We also show that our model design is applicable to nested named entity recognition task, where it performs on par with state-of-the-art approach designed for that task. Finally, we demonstrate that our approach is 2-3.5 times faster than the sequence-to-sequence model at inference time.

==> tables/top-stats.tex <==
\small
\centering
\begin{tabular}[t]{ccc|cccccc}
\toprule
Dataset & Domain & SPIS & Train & Valid & Test & Intent & Slots & Flat$\%$  \\
\midrule
{\tt TOP} & & & $28414$ & $4032$ & $8241$ & $25$ & $36$ & $61\%$ \\
\midrule
\multirow{2}{*}{{\tt TOPv2}} & \multirow{2}{*}{\textit{Reminder}} & $25$ & $493$ & $337$ & \multirow{2}{*}{$5767$} & \multirow{2}{*}{$19$} & \multirow{2}{*}{$32$} & \multirow{2}{*}{$79\%$} \\ 
& & $500$ & $4788$ & $2526$ & & & & \\ \midrule
\multirow{2}{*}{{\tt TOPv2}} & \multirow{2}{*}{\textit{Weather}} & $25$ & $176$ & $147$ & \multirow{2}{*}{$5682$} & \multirow{2}{*}{$7$} & \multirow{2}{*}{$11$} & \multirow{2}{*}{$100\%$} \\
& & $500$ & $2372$ & $2667$ & & & & \\

\bottomrule
\end{tabular}
\caption{Statistics of {\tt TOP} and {\tt TOPv2} datasets. \textit{SPIS} stands for samples for each intent and slot label. \textit{Intent} stands for number of intents. \textit{Slots} stands for number of slots. Flat$\%$ stands for the fraction of the dataset containing flat queries. }
